Infinite-Dimensional Feature Interaction

The past neural network design has largely focused on feature representation space dimension and its capacity scaling (e.g., width, depth), but overlooked the feature interaction space scaling. Recent advancements have shown shifted focus towards element-wise multiplication to facilitate higher-dimensional feature interaction space for better information transformation. Despite this progress, multiplications predominantly capture low-order interactions, thus remaining confined to a finite-dimensional interaction space. To transcend this limitation, classic kernel methods emerge as a promising solution to engage features in an infinite-dimensional space. We introduce InfiNet, a model architecture that enables feature interaction within an infinite-dimensional space created by RBF kernel. Our experiments reveal that InfiNet achieves new state-of-the-art, owing to its capability to leverage infinite-dimensional interactions, significantly enhancing model performance.

==> _txt/_hist/1_Introduction.tex <==
\section{Introduction}

During the past decades, the machine learning community has turned from traditional machine learning algorithm almost exclusively to neural networks. 
    Although the model evolutionary, both traditional machine learning and deep learning agree that the dimension of feature representation space matters. 
        This can be illustrated by the introduction of ensemble~\cite{opitz1999popular,breiman2001random} and kernel methods~\cite{fan1995local,scholkopf1997comparing} in the traditional models, as well as in the increasing width and depth of the deep models~\cite{krizhevsky2012imagenet,he2016deep}.
At the same time, we note that in practice, due to the a priori knowledge of the deep semantic connections between data dimensions, the models we used are often not simple multi-layer perceptrons (MLPs), but models with specific architectures to capture global or local feature interactions. 
    
 
 These feature interactions such as features attention mechanism~\cite{vaswani2017attention,bai2021attentions,dosovitskiy2020image}, gated aggregation~\cite{li2022efficient,rao2022hornet,yang2022focal}, and quadratic neurons~\cite{xu2023quadranet,fan2023one,xu2022quadralib}, are attributed to element-wise multiplication~\cite{ma2024rewrite}. This multiplication between elements is noted as an expansion for the feature interaction space and, at a more macroscopic level, a approximation of the kernel methods~\cite{ma2024rewrite}. 
    This is due to the fact that, by this multiplication operation between elements, we construct an implicit quadratic space $\mathcal{Q}$ with of degrees of freedom $\frac{n^2}{2}$ from the original feature vector space $\mathcal{V}$ with $n$-dimensions, by means of the quadratic form. 
However, the implicit feature interaction space thus constructed still only captures simple quadratic interactions between feature elements, and thus more complex and higher level interactions are still not modeled. 

The inherent challenge of capturing high-level interactions in high-dimensional spaces lies in maintaining low computational complexity. Architectural adjustments to existing neural networks bring only a limited expansion of the feature interaction space at the cost of parallelizability~\cite{rao2022hornet} and computational complexity~\cite{li2022efficient}.

\begin{center}
    \textit{How can we efficiently extend interactions to a high-dimensional space?}
\end{center}

%The deeper reason for this trend is the theoretical guarantees given by the formulation of the Universal Approximation Theorem~\cite{hornik1990universal} for neural networks and the simplicity of multi-layer perceptrons (MLP). The Universal Approximation Theorem tells us that in order to fit a function with higher accuracy, we need to add more neurons to the hidden layer, which leads to wider and deeper network architecture today. 

==> _txt/_hist/1_Introduction__Xiang_Chen_s_conflicted_copy_2024-05-17_.tex <==
\section{Introduction}
Over the past decades, the focus of the machine learning community has largely shifted from traditional algorithms to neural networks. Despite these evolutionary changes, a common understanding persists across both traditional machine learning and deep learning: the dimensionality of the feature representation space is critical. This is evidenced by the adoption of ensemble techniques~\cite{opitz1999popular,breiman2001random} and kernel methods~\cite{fan1995local,scholkopf1997comparing} in traditional machine learning approaches, as well as by the increased width and depth in neural network architectures~\cite{krizhevsky2012imagenet,he2016deep}.

Moreover, in practical applications, the models employed often transcend simple multi-layer perceptrons (MLPs), incorporating specialized architectures designed to capture both global and local feature interactions. Noteworthy among these are attention mechanisms~\cite{vaswani2017attention,bai2021attentions,dosovitskiy2020image}, gated aggregation~\cite{li2022efficient,rao2022hornet,yang2022focal}, and quadratic neurons~\cite{xu2023quadranet,fan2023one,xu2022quadralib}. These interactions, facilitated through element-wise multiplication~\cite{ma2024rewrite}, enhance the feature interaction space and offer a macroscopic approximation to kernel methods. By employing this multiplication, an implicit interactive quadratic space $\mathcal{Q} = \text{span}\left(x_1^2, x_1x_2,\cdots, x_{n-1}x_n, x_n^2\right)$ with degrees of freedom $\frac{n^2+n}{2}$ is constructed from the original $n$-dim vector space $\mathcal{V} =\text{span}\left(x_1,x_2,\cdots,x_n\right)$ using a quadratic form $\mathbf x^TW_a^TW_b\mathbf x$ (equals to $\langle W_a\mathbf{x},W_b\mathbf x\rangle$) ~\cite{ma2024rewrite}. Therefore, the next layer feature is generated with the linear combination on the feature interaction space $\mathcal Q$ instead of on the feature representation space $\mathcal V$.


However, this newly formed feature interaction space captures still only basic quadratic interactions, leaving more complex and high-level interactions~(e.g. $x_1^3x_2^2$, $\lim\limits_{k\to \infty} x_1^k$) unmodeled, where exists a great opportunity.
%$\lim\limits_{k\to \infty} x_1^k$
%$\langle W_a\mathbf{x},W_b\mathbf x\rangle$
One of the inherent challenges in modeling high-level interactions within high-dimensional spaces is maintaining manageable computational complexity. Architectural enhancements in neural networks often result in only marginal increases in the capacity for feature interactions, at the cost of parallelizability~\cite{rao2022hornet} and computational overhead~\cite{li2022efficient,dosovitskiy2020image}. %It's an open question that:

\begin{center}
\textit{How can we efficiently extend interactions to a high-dimensional space?}
\end{center}

Inspired by the traditional machine learning community, we propose an approach that introduces kernel methods for feature interaction in neural networks. We define a set of feature interactions between features $W_a\mathbf{x}$ and $W_b\mathbf x$ with a kernel function $\mathit K(W_a\mathbf{x},W_b\mathbf x)$ instead of the element-wise multiplication.
From there, the feature interaction space is defined by the inner product on the Reproducing Kernel Hilbert Space (RKHS)~\cite{aronszajn1950theory} $\mathcal H$ constituent with the kernel function $\mathit K(\cdot,\cdot)$.

In this paper, we propose KerNet, a novel family of neural networks that generate feature representations hierarchically by performing information aggregation on an infinite-dimensional feature interaction space.
    KerNet performs the interaction between multiple branches of the feature's information proper by the introduction of Radial Basis Function (RBF) kernel~\cite{musavi1992training}.
        The RBF kernel maps feature interactions to an infinite-dimensional space, so that the information transfer flow within the neural network always takes place between infinite-dimensional spaces.
        Thereby, a neural network activated by ReLU is not only mining the linear pathway from the original input to the output, but each layer in the multi-layer architecture of the neural network is mining the nonlinear correlations of arbitrary order between different positions in the previous layer feature.

\textbf{Contributions.} We make the following contributions:
\begin{itemize}
    \item We reveal that the shift of the information transfer flow within neural networks from feature representation space to feature interaction space is a key factor in embedding feature information into high-dimensional space and therefore improving model performance.
 %   \item We propose a method of expanding the dimension of the feature interaction space using kernel methods. Utilizing this super-high-dimensional feature interaction, neural network's can effectively model the complex implicit correlations of features in each layer.
    \item We propose KerNet, a novel variant of neural networks expanding the feature interaction space to infinite dimension with RBF kernel, that can effectively model the complex implicit correlations of features in each layer.
\end{itemize}


==> _txt/_hist/1_Introduction_legacy.tex <==
\section{Introduction}

Over the past few years, the architecture of state-of-the-art vision neural networks has undergone a significant evolution, transitioning from simple neural interactions such as convolution \cite{lecun1998gradient} and MLP \cite{khotanzad1998application} to embrace high-order element-wise interactions \cite{rao2022hornet}. Meanwhile, the widespread adoption of a depth-width separable design in most models \cite{howard2017mobilenets,dosovitskiy2020image,liu2022convnet} has notably enhanced model efficiency. However, the prevalent use of depth-width separable designs in contemporary networks like ViT \cite{dosovitskiy2020image} and HorNet \cite{rao2022hornet} confines these element-wise interactions within a low-dimensional space, thus failing to fully exploit their potential to explore more non-linearity in high-dimensional space. This design approach leads to high-order element-wise neural interactions occurring in a channel-by-channel and pixel-to-pixel manner, thereby restricting the maximum interaction order between pixels to a low level (3 for ViT and $n$ in $g_{n}\text{Conv}$ for HorNet).

The inherent challenge of capturing high-order interactions in high-dimensional spaces lies in maintaining low computational complexity. When employing a linear transformation to expand the space, the computational complexity would be $O(nr)$, where $n$ and $r$ represent the dimensions of features before and after expansion, respectively. HorNet~\cite{rao2022hornet} constrains the computational complexity and parameter count associated with high-order interactions by exponentially reducing the number of channels. MogaNet~\cite{li2022efficient} distributes high-order interactions across various components of the network. These endeavors minimize computational requirements while preserving high-order interactions, however, constrict the feasible space of high-order interaction to a small extent.

\begin{center}
    \textit{How can we efficiently extend interactions to a high-dimensional space?}
\end{center}

An intuitive approach to address this query is through kernel methods~\cite{scholkopf1997comparing,fan1995local}, extensively utilized in traditional machine learning techniques such as Support Vector Machines and Principal Component Analysis. Kernel methods implicitly learn a mapping from the original low-dimensional space to a higher-dimensional one, obviating the need for explicit parameterized transformations that escalate computational and memory demands. While kernel methods are commonly employed as a substitute for inner products between sets of data points or features, such inner products are rare in neural networks due to their reliance on parameterized weight matrices multiplied with data.

%Among the many high-order neural interaction methods, quadratic neural networks~\cite{xu2023quadranet,xu2022quadralib} inherently provide high-order neural interactions and accumulate inner products in a neural format. Consequently, quadratic neurons serve as a conducive platform for employing kernel methods. Moreover, the incorporation of polynomials within quadratic neural networks enables model initialization through weight acquisition from a pre-trained standard neural network.

In this study, we exploit the characteristics of quadratic neural networks to expand the inherent high-order neural interactions within the quadratic term of quadratic neurons into a high-dimensional space using kernel methods, thereby establishing a novel family of neural networks termed InfiNet. In addition to extending the space for high-order interactions, InfiNet maintains a variety of advantages, including \textit{Input-adaptive Weights}, \textit{Long-range Dependency Capture}, \textit{Extensibility}, \textit{Scalability}, and \textit{Translation Equivalence}.

Furthermore, We treat the quadratic term in InfiNet as an adapter and initialize it by acquiring weights from ConvNeXt~\cite{liu2022convnet}, which has undergone sufficient pre-training, thus circumventing redundant, resource-intensive pre-training for sustainable and eco-friendly machine learning.


We undertake comprehensive experiments on ImageNet classification~\cite{deng2009imagenet}, MS COCO object detection~\cite{lin2014microsoft}, and ADE20K semantic segmentation~\cite{zhou2017scene} to validate the efficacy of our propose InfiNets. 
%实验写完以后补一点实验数据的总结




\begin{comment} 
HorNet~\cite{rao2022hornet} keeps the computation and number of parameters for high-order interactions within an acceptable limit by decreasing the number of channels exponentially. MogaNet~\cite{li2022efficient} spreads the high-order in different components of the network. These attempts to reduce the amount of computation, while maintaining high-order interactions, compress the space in which they can be exerted to a very small extent.

\begin{center}
    \textit{How should we efficiently expand the interaction to a high-dimensional space?} 
\end{center}

An intuitive approach to answer this question is kernel methods~\cite{scholkopf1997comparing,fan1995local} that have been widely adopted in the traditional machine learning methods such as Support Vector Machine and Principal Component Analysis. Kernel methods learn an implicit mapping from original low dimensional space to a high dimensional one, avoiding an explicit parameterized transformation that increase the computing and memory loads. The kernel methods are generally adopted in substitute of inner product between two sets of data points or features, however such inner product rarely happens in the neural networks. This is due to the fact that neural networks is in the scheme that multiply parameterized weight matrix with data. 

We notice that the quadratic neural networks~\cite{xu2023quadranet,xu2022quadralib} it self not only provide the high-order neural interaction but also accumulate an inner product in the neural format. This makes the quadratic neuron itself provide a good platform for exerting the kernel methods. At the same time, the quadratic neural network itself incorporates a polynomial, which makes it possible to initialize the model by obtaining weights from a standard neural network that has been trained. 



In this paper, we leverage such characterization of quadratic neural networks to expanding the endogenous high-order neural interaction in the quadratic term of quadratic neuron into a high-dimensional space with kernel methods, and thus build a new family of neural networks called \textbf{Q}uadratic \textbf{K}ernel \textbf{A}dapted Networks~(InfiNet). We We treat the quadratic term in InfiNet as an adapter and then initialize the InfiNet by obtaining weights from ConvNeXT~\cite{liu2022convnet} that has been sufficiently pre-trained, as a way to avoid repetitive, resource-consuming pre-training, for an sustainable and green machine learning.

\end{comment}



==> _txt/_hist/3_Method.tex <==
\section{Methods}
\subsection{Quadratic Neural Networks}
We start from a quadratic neuron with quadratic weight matrix $W_q$ of rank $k$ with output $f_\text{quad}(X)$:

\begin{equation}
    y_\text{quad}(X) = \sigma(X^TW_qX+W_cX+b) = \sigma(X^TW_a^TW_bX+W_cX+b),
\end{equation}
where the input with dimension $n$, $W_q \in \mathbb{R}^{n \times n}$ is a symmetric matrix, $W_a$, $W_b \in \mathbb{R}^{n\times k}$, and $\sigma(\cdot)$ is the activation function. We convert the quadratic forms $H(\cdot)$ defined by $W_q$ to inner products:

\begin{equation}
    H(X)= X^TW_qX = X^TW_a^TW_bX = <W_aX,W_bX>,
\end{equation}

where $<\cdot,\cdot>$ indicates inner product. Thus a single Quadratic Neuron can be expressed as:
\begin{equation}
    y_\text{quad}(X) = \sigma(<W_aX,W_bX>+W_cX+b)
\end{equation}
When we port quadratic neural networks to convolutional operations, the $i_\text{th}$ element of the convolution output $y_\text{quad\_conv}(\mathbf x)$ is calculated as:
\begin{equation}
    y_\text{quad\_conv}(\mathbf x)_i = \sigma(<\mathbf{w}_a\mathbf{x}_{(i)},\mathbf w_b\mathbf x_{(i)}>+\mathbf{w}_c\mathbf x_{(i)}),
\end{equation}

where $\mathbf w_a$ and $\mathbf w_b$ are two groups of different and independent convolution filters with number of $k$, and $\mathbf w_c$ is a single convolution filter , $\mathbf x_{(i)}$ represents the convolution operation's receptive field of the $i_\text{th}$ element of the output. Then $\mathbf{w}_a\mathbf{x}_{(i)}$ and $\mathbf{w}_b\mathbf{x}_{(i)}$ are with the shape of $k\times 1$ respectively.

\subsection{Inner Product Substitution with Kernel Methods}


Given the mathematical expression of the quadratic form  $X^TW_a^TW_bX$, which is the inner product of the linear transformations of the two inputs $W_aX$ and $W_bX$~\cite{kurepa2006quadratic}. We denote the inner product as $<W_aX,W_bX>$.

We replace the inner product $<W_aX,W_bX>$ defined by the quadratic term with the kernel function $\mathcal{K}(W_aX,W_bX)$. As a kernel, $\mathcal{K}$ corresponds to an inner product in a feature space based on some mapping $\phi$. Therefore, Kernel Methods maps the inner product defined by the original quadratic adapter through an implicit nonlinear mapping:
\begin{equation}
    \mathcal{K}(W_aX,W_bX) = <\phi(W_aX),\phi(W_bX)>
\end{equation}

We consider the following kernel functions:

(1) Polynomial Kernel: 
\begin{equation}
    \mathcal{K}_{\text{Polynomial}}(\mathbf{x},\mathbf{x}') = (\mathbf{x}^T\mathbf{x}'+c)^d
\end{equation}

(2) Radial Basis Function Kernel:
\begin{equation}
\mathcal{K}_{\text{RBF}}\left(\mathbf{x}, \mathbf{x}^{\prime}\right)=\exp \left(-\frac{\left\|\mathbf{x}-\mathbf{x}^{\prime}\right\|^2}{2 \sigma^2}\right)
\end{equation}

Polynomial Kernel maps the feature representations to an high-dimensional space that is span of $\{\mathbf{x}^d,\mathbf{x'}^d,\mathbf{x}^{d-1}\mathbf{x'},\cdots,\mathbf{x},1\}$, while RBF Kernel maps them to an infinite-dimensional space, given the fact that: 
\begin{equation}
\exp \left(-\frac{1}{2}\left\|\mathbf{x}-\mathbf{x}^{\prime}\right\|_2^2\right)=\sum_{j=0}^{\infty} \frac{\left(\mathbf{x}^{\top} \mathbf{x}^{\prime}\right)^j}{j !} \exp \left(-\frac{1}{2}\|\mathbf{x}\|_2^2+\left\|\mathbf{x}^{\prime}\right\|_2^2\right)
%\exp \left(-\frac{1}{2}\left\|\mathbf{x}-\mathbf{x}^{\prime}\right\|_2^2\right)=\sum_{j=0}^{\infty} \frac{\left(\mathbf{x}^{\top} \mathbf{x}^{\prime}\right)^j}{j !} \exp \left(-\frac{1}{2}\|\mathbf{x}\|_2^2\right) \exp \left(-\frac{1}{2}\left\|\mathbf{x}^{\prime}\right\|_2^2\right).
\end{equation}
The introduction of the kernel approach allows us to further model the features of adapter, which were originally modeled only up to the quadratic level, into the higher order neural interaction space with minimum cost. Thus exploring divisibility of features in high order spaces.

==> _txt/_hist/ADE20K.tex <==
\begin{table}
  \caption{\textbf{ADE20K Segmentation}}
  \label{tab:segmentation}
  \centering
  \begin{tabular}{lllll}
    \toprule
%    \multicolumn{2}{c}{Part}                   \\
%    \cmidrule(r){1-2}
    Model     & mIoU$^\text{ss}$  & mIoU$^\text{ms}$    & Params(M)  & FLOPs(G)  \\
    \midrule
    InfiNet-T & 46.7  & 47.4& 50  & 924 \\
    InfiNet-S    & 49.4 & 49.9  & 78&  1002 \\
    InfiNet-B     & 50.2 &  50.9& 105& 1111 \\
    InfiNet-XL*  & 54.6  & 54.8  &  253 & 2474 \\
    \bottomrule
  \end{tabular}
\end{table}
